Modeling Black-Box Components with Probabilistic Synthesis

This paper is concerned with synthesizing programs based on black-box oracles: we are interested in the case where there exists an executable implementation of a component or library, but its internal structure is unknown. We are provided with just an API or function signature, and aim to synthesize a program with equivalent behavior. To attack this problem, we detail Presyn: a program synthesizer designed for flexible interoperation with existing programs and compiler toolchains. Presyn uses high-level imperative control-flow structures and a pair of cooperating predictive models to efficiently narrow the space of potential programs. These models can be trained effectively on small corpora of synthesized examples. We evaluate Presyn against five leading program synthesizers on a collection of 112 synthesis benchmarks collated from previous studies and real-world software libraries. We show that Presyn is able to synthesize a wider range of programs than each of them with less human input. We demonstrate the application of our approach to real-world code and software engineering problems with two case studies: accelerator library porting and detection of duplicated library reimplementations.

==> overview.tex <==
% This section gives a brief summary of the structure of this paper. In
% \Cref{sec:contribs} we detail our contributions to this area of study and show
% how they relate to the existing body of work.  \Cref{sec:implementation} details
% the synthesis techniques used by our implementation (\presyn{}). Then, in
% \Cref{sec:setup} we describe an experimental setup to evaluate \presyn{} against
% other state-of-the-art synthesizers on a common set of problems.
% \Cref{sec:results} discusses the results of these experiments. Finally, in
% \Cref{sec:related} we discuss related work, and in \Cref{sec:conclusion} we
% summarise the contributions of this paper and identify potential areas for
% future work.

